Enabling Data Confidentiality with Public Blockchains

Blockchain technology is apt to facilitate the automation of multi-party cooperations among various players in a decentralized setting, especially in cases where trust among participants is limited. Transactions are stored in a ledger, a replica of which is retained by every node of the blockchain network. The operations saved thereby are thus publicly accessible. While this aspect enhances transparency, reliability, and persistence, it hinders the utilization of public blockchains for process automation as it violates typical confidentiality requirements in corporate settings. To overcome this issue, we propose our approach named Multi-Authority Approach to Transaction Systems for Interoperating Applications (MARTSIA). Based on Multi-Authority Attribute-Based Encryption (MA-ABE), MARTSIA enables read-access control over shared data at the level of message parts. User-defined policies determine whether an actor can interpret the publicly stored information or not, depending on the actor's attributes declared by a consortium of certifiers. Still, all nodes in the blockchain network can attest to the publication of the (encrypted) data. We provide a formal analysis of the security guarantees of MARTSIA, and illustrate the proof-of-concept implementation over multiple blockchain platforms. To demonstrate its interoperability, we showcase its usage in ensemble with a state-of-the-art blockchain-based engine for multi-party process execution, and three real-world decentralized applications in the context of NFT markets, supply chain, and retail.

==> addon/glossary.tex <==
\RequirePackage{xspace}

\newacronym[\glslongpluralkey={Distributed Ledger Technologies}]{dlt}{DLT}{Distributed Ledger Technology}
\newcommand{\DLT}[0] {\Gls{dlt}\xspace}
\newcommand{\DLTs}[0] {\Glspl{dlt}\xspace}

\newacronym{avm}{AVM}{Algorand Virtual Machine}
\newcommand{\AVM}[0] {\Gls{avm}\xspace}
\newacronym{evm}{EVM}{Ethereum Virtual Machine}
\newcommand{\EVM}[0] {\Gls{evm}\xspace}

\newacronym{dapp}{DApp}{Decentralized Application}
\newcommand{\DApp}[0] {\Gls{dapp}\xspace}
\newcommand{\DApps}[0] {\Glspl{dapp}\xspace}

%\newacronym{gasu}{GU}{gas unit}
%\newcommand{\GasU}[0] {\Gls{gasu}\xspace}

\newacronym{nft}{NFT}{Non-Fungible Token}
\newcommand{\NFT}[0] {\Gls{nft}\xspace}
\newcommand{\NFTs}[0] {\Glspl{nft}\xspace}

\newacronym{ipfs}{IPFS}{InterPlanetary File System}
\newcommand{\IPFS}[0] {\Gls{ipfs}\xspace}

\newacronym{p2p}{P2P}{peer-to-peer}
\newcommand{\PtoP}[0] {\Gls{p2p}\xspace}

\newacronym{abe}{ABE}{Attribute-Based Encryption}
\newcommand{\ABE}[0] {\Gls{abe}\xspace}

\newacronym{maabe}{MA-ABE}{Multi-Authority Attribute-Based Encryption}
\newcommand{\MAABE}[0] {\Gls{maabe}\xspace}


\newacronym{cpabe}{CP-ABE}{Ciphertext-Policy Attribute-Based Encryption}
\newcommand{\CPABE}[0] {\Gls{cpabe}\xspace}

\newacronym{ssl}{SSL}{Secure Sockets Layer}

\newacronym{dht}{DHT}{Distributed Hash Table}
\newcommand{\DHT}[0] {\Gls{dht}\xspace}

\newacronym{mpc}{MPC}{Multi-party Computation}
\newcommand{\MPC}[0] {\Gls{mpc}\xspace}

\newglossaryentry{box}{ %
  name={Box},
  description={authority intialisation storage box},
  first={\glsentrydesc{box} (henceforth, \glsentrytext{Box} for short)},
  plural={Boxes},
  firstplural={\glsentrydesc{box}es (henceforth, \glsentryplural{box} for short)}
}
\newcommand{\abox}[0] {\gls{box}\xspace}
\newcommand{\aboxes}[0] {\glspl{box}\xspace}

\newglossaryentry{rloc}{ %
	name={resource locator},
	description={a generic term to denote content-based links obtained via hashing (e.g., the IPFS link)},
}
\def\rloc{\gls{rloc}\xspace}
\def\Rloc{\Gls{rloc}\xspace}
\def\GasU{GU\xspace}

\newacronym{cpmaabe}{CP-MA-ABE}{Ciphertext-Policy Multi-Authority Attribute-Based Encryption}
\newcommand{\CPMAABE}[0] {\Gls{cpmaabe}\xspace}

%
\def\DOwner{Data Owner\xspace}
\def\AttCert{Attribute Certifier\xspace}
\def\Reader{Reader\xspace}
\def\SC{Smart Contract\xspace}
\def\MeC{Message Contract\xspace}
\def\AtC{Attribute Certifier Contract\xspace}
\def\AutC{Authority Contract\xspace}
\def\RSAC{RSA Public Key Contract\xspace}
\def\Auth{Authority\xspace}
\def\Auths{Authorities\xspace}
\def\DStore{Data Store\xspace}

\newacronym{dk}{\textsl{dk}}{decryption key}
\newacronym{fdk}{\textsl{fdk}}{final decryption key}
\def\dk{\gls{dk}\xspace}
\def\fdk{\gls{fdk}\xspace}

==> addon/macros-crypto.tex <==
\RequirePackage{mathtools}
\RequirePackage{amsmath}

\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
%\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}

\renewcommand{\S}{Sec. }
\newcommand{\cind}{\approx_c}
\newcommand{\sind}{\approx_s}
\newcommand{\aux}{z}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\alg}[1]{\mathsf{#1}}
\newcommand{\bin}{\{0,1\}}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\secpar}{\lambda}
\newcommand{\rv}[1]{\mathbf{#1}}
\newcommand{\poly}{\mathtt{poly}}
\newcommand{\negl}{\mathtt{negl}}
\newcommand{\continue}{\mathtt{continue}}
\newcommand{\abort}{\mathtt{abort}}
\newcommand{\out}{\mathtt{output}}
\newcommand{\shares}{\sigma}

\newcommand{\cS}{\set{S}}
\newcommand{\adv}[3]{\mathtt{Adv}_{#1}^{#2} (#3)}
\newcommand{\oracle}{\mathcal{O}}
\newcommand{\unifdistr}{\mathbf{U}}
\newcommand{\distr}{\mathbf{D}} 
\newcommand{\CD}[4]{\mathbb{CD}_{#1}(#3, #4) \leq #2}
\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
\newcommand{\advA}{\alg{A}}
\newcommand{\advS}{\alg{S}}
\newcommand{\gamesym}{\mathbf{G}}
\newcommand{\rndsample}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\distrsample}{\leftarrow\!\mathsmaller{\distr}\ }
\newcommand{\msb}[2]{\mathsf{msb}_{#2}({#1})}
\newcommand{\lsb}[2]{\mathsf{lsb}_{#2}({#1})}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\advD}{\mathsf{D}}
\newcommand{\SD}[1]{\mathbb{SD}\left(#1\right)}
\newcommand{\Prob}[1]{\mathbb{P}\left[#1\right]}


\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

%
% Calligraphic letters
%

\newcommand{\calA}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\calB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\calC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\calD}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\calE}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\calF}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\calG}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\calH}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\calI}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\calK}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\calL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\calM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\calN}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\calO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\calP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\calR}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\calS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\calT}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\calU}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\calV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\calW}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\calX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}\xspace}


% Bold Face Letters

\newcommand{\bfA}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\bfB}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\bfC}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\bfD}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\bfE}{\ensuremath{\mathbf{E}}\xspace}
\newcommand{\bfF}{\ensuremath{\mathbf{F}}\xspace}
\newcommand{\bfG}{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\bfH}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\bfI}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\bfJ}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\bfK}{\ensuremath{\mathbf{K}}\xspace}
\newcommand{\bfL}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\bfM}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\bfN}{\ensuremath{\mathbf{N}}\xspace}
\newcommand{\bfO}{\ensuremath{\mathbf{O}}\xspace}
\newcommand{\bfP}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\bfQ}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\bfR}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\bfS}{\ensuremath{\mathbf{S}}\xspace}
\newcommand{\bfT}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\bfU}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\bfV}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\bfW}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}\xspace}

\newcommand{\advB}{\mathsf{B}}
\newcommand{\pk}{\mathit{pk}}
\newcommand{\sk}{\mathit{sk}}

\newcommand{\roundreset}{c}
\newcommand{\inp}{x}
\newcommand{\rand}{\omega}
\newcommand{\nnum}{n}
\newcommand{\thr}{t}
\newcommand{\func}{f}
\newcommand{\gunc}{g}
\newcommand{\round}{r}
\newcommand{\nextmsg}{\psi}
\newcommand{\trans}{\tau}
\newcommand{\msg}{m}
\newcommand{\Rel}{R}
\newcommand{\Lang}{L}
\newcommand{\stm}{x}
\newcommand{\NICom}{\alg{Commit}}
\newcommand{\com}{\gamma}
\newcommand{\coms}{C}
\newcommand{\open}{\delta}
\newcommand{\share}{\mathsf{Share}}
\newcommand{\recon}{\mathsf{Recon}}

\newcommand{\party}{\alg{P}}
\newcommand{\vparty}{\mathbb{P}}
\newcommand{\REAL}{\rv{REAL}}
\newcommand{\IDEAL}{\rv{IDEAL}}
\newcommand{\HYBRID}{\rv{HYBRID}}
\newcommand{\HYB}{\rv{H}}
\newcommand{\coins}{\mathsf{coins}}

\newcommand{\setup}{\alg{Setup}}
\newcommand{\Prove}{\alg{Prove}}
\newcommand{\Ver}{\alg{Ver}}
\newcommand{\nip}{\phi}
\newcommand{\crs}{\sigma}
\newcommand{\tk}{\zeta}
\newcommand{\xtk}{\xi}
\newcommand{\ZKSim}{\alg{ZKSim}}
\newcommand{\KExt}{\alg{KExt}}
\newcommand{\LR}{\alg{LR}}
\newcommand{\BAD}{\rv{BAD}}
\newcommand{\wit}{w}
\newcommand{\cph}{c}
\newcommand{\sgn}{\sigma}
\newcommand{\sfE}{\mathsf{E}} 
\newcommand{\Open}{\ensuremath{\mathsf{Open}}}

\newcommand{\Enc}{\ensuremath{\mathsf{Enc}}}
\newcommand{\Dec}{\ensuremath{\mathsf{Dec}}}
\newcommand{\Gen}{\ensuremath{\mathsf{Gen}}}
\newcommand{\Eval}{\ensuremath{\mathsf{Eval}}}
\newcommand{\Vrfy}{\ensuremath{\mathsf{Check}}}
\newcommand{\VRF}{\ensuremath{\mathsf{VRF}}}
\newcommand{\Hash}{\ensuremath{\mathsf{Hash}}}
\newcommand{\query}{\ensuremath{\mathtt{query}}}
\newcommand{\Tx}{\ensuremath{\mathsf{Tx}}}
\newcommand{\tx}{\ensuremath{\mathsf{tx}}}
\newcommand{\hyb}{\ensuremath{\mathbf{Hyb}}}
\newcommand{\game}{\ensuremath{\mathbf{G}}}
\newcommand{\vk}{\mathit{vk}}
\newcommand{\idf}{\func^{\sf pct}}
\newcommand{\Sign}{\ensuremath{\mathsf{Sign}}}
\newcommand{\Verify}{\ensuremath{\mathsf{Verify}}}

\newcommand{\UpdateState}{\mathsf{UpdateState}}
\newcommand{\GetRecords}{\mathsf{GetRecords}}
\newcommand{\Broadcast}{\mathsf{Broadcast}}
\newcommand{\formalst}{\mathit{st}}
\newcommand{\Consistent}{\mathsf{Consistent}}
\newcommand{\Bchain}{\mathcal{B}}
\newcommand{\block}{\beta}
\newcommand{\mes}{M}
\newcommand{\view}{\mathit{view}}
\newcommand{\Exec}{\rv{EXEC}}
\newcommand{\states}{\mathbf{ST}}
\newcommand{\blocks}{\mathsf{blocks}}
\newcommand{\bigO}{O}
\newcommand{\bround}{r}
\newcommand{\liveness}{\mathsf{Live}}
\newcommand{\ctr}{r}

\newcommand{\ek}{\mathit{ek}}
\newcommand{\formaldk}{\mathit{dk}}
\newcommand{\quality}{\mathsf{Quality}}
\newcommand{\advZ}{\alg{Z}}

\newcommand{\rushthr}{\varphi}
\newcommand{\prunethr}{k}
\newcommand{\wait}{w}

\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cM}{\mathcal{M}}

\newcommand{\ctx}{c}

\newcommand{\Bad}{\BAD}

\newcommand{\Func}{\ensuremath{\mathcal{F}}}
\newcommand{\Sim}{\ensuremath{\mathsf{S}}}
\newcommand{\cominput}{\ensuremath{\mathsf{input}}}
\newcommand{\return}{\ensuremath{\mathsf{return}}}
\newcommand{\extra}{\ensuremath{\mathsf{extra}}}
\newcommand{\extrapay}{\ensuremath{\mathsf{extrapay}}}
\newcommand{\sendback}{\ensuremath{\mathsf{sendback}}}
\newcommand{\payback}{\ensuremath{\mathsf{payback}}}
\newcommand{\prize}{\ensuremath{\mathsf{prize}}}
\newcommand{\comoutput}{\ensuremath{\mathsf{output}}}
\newcommand{\compenalty}{\ensuremath{\mathsf{penalty}}}
\newcommand{\lock}{\ensuremath{\mathsf{lock}}}
\newcommand{\FuncML}{\ensuremath{\Func^*_{ML}}}
\newcommand{\FuncSC}{\ensuremath{\Func_\mathsf{SC}}}
\newcommand{\locked}{\ensuremath{\mathsf{locked}}}
\newcommand{\redeem}{\ensuremath{\mathsf{redeem}}}
\renewcommand{\wit}{\ensuremath{w}}
\newcommand{\payout}{\ensuremath{\mathsf{payout}}}
\newcommand{\ret}{\ensuremath{\mathsf{return}}}
\newcommand{\FuncLOT}{\ensuremath{\mathcal{F}^*_\mathsf{lot}}}
\newcommand{\PayDeposit}{\ensuremath{\mathsf{PayDeposit}}}
\newcommand{\Commit}{\ensuremath{\mathsf{Commit}}}
\newcommand{\Compute}{\ensuremath{\mathsf{Compute}}}
\newcommand{\PutMoney}{\ensuremath{\mathsf{PutMoney}}}
\newcommand{\picomp}{\pi'}
\newcommand{\pibc}{\pi'_{bc}}
\newcommand{\pifair}{\pi_\mathsf{fair}}
\newcommand{\rushing}{hasty}
\newcommand{\Rushing}{Hasty}
\newcommand{\nonrushing}{non-hasty}
\newcommand{\Nonrushing}{Non-hasty}

\newcommand{\pitr}{\pi_\mathsf{TR}}

\newcommand{\authsetup}{\alg{AuthSetup}}
\newcommand{\enc}{\alg{Enc}}
\newcommand{\kgen}{\alg{KGen}}
\newcommand{\dec}{\alg{Dec}}
\newcommand{\params}{\ensuremath{\mathit{pp}}}

\newcommand{\pol}{\mathbb{A}}
\newcommand{\attr}{\alpha}
\newcommand{\id}{\mathsf{id}}
\newcommand{\auths}{\mathcal{T}}
\newcommand{\cipher}{c}
\newcommand{\attrs}{\mathcal{U}}
\newcommand{\idents}{\mathcal{I}}
\newcommand{\auth}{\psi}
\newcommand{\msgspace}{\mathcal{M}}
\newcommand{\corr}{\mathcal{C}}
\newcommand{\etal}{{et~al.}}

\newcommand{\cQuery}{\mathcal{Q}}
\newcommand{\polpred}{\mathsf{T}}


\newcommand{\FuncTR}{\mathcal{F}_\mathsf{TR}}
\newcommand{\FuncBC}{\mathcal{F}_\mathsf{BC}}
\newcommand{\dataowner}{D}
\newcommand{\reader}{R}
\newcommand{\readers}{\mathcal{R}}
\newcommand{\storemessage}{\textsc{StoreMessage}}
\newcommand{\messagestored}{\textsc{MessageStored}}
\newcommand{\readmessage}{\textsc{ReadMessages}}
\newcommand{\inputcom}{\textsc{Input}}
\newcommand{\outputcom}{\textsc{Output}}
\newcommand{\post}{\textsc{Post}}
\newcommand{\readcom}{\textsc{Read}}
\newcommand{\dict}{\mathsf{dict}}
\newcommand{\messages}{\mathsf{msg}}
\newcommand{\parties}{\mathcal{P}}
\newcommand{\chain}{\mathsf{chain}}
\newcommand{\counter}{\mathsf{ctr}}


\newcommand{\formalMAABE}{\mathsf{ABE}}
\newcommand{\SIG}{\mathsf{SIG}}
\newcommand{\PKE}{\mathsf{PKE}}



\newcommand{\un}[1]{{\color{red} #1}}

\newcommand{\Comment}[2][red]{\marginpar{
		\fcolorbox{#1}{white}{\parbox{.8in}{
				\color{#1} \small \sf  #2 }}}}
\newcommand{\mcomment}[2]{\textcolor{red}{#1}\Comment{#2}}
\newcommand{\TODO}[2][\relax]{\noindent\mcomment{#2}{#1 TODO}}
\newcommand{\mytodo}[2]{\mcomment{ #1 }{#2 TODO}}
\newcommand{\ucomment}[3]{\par\noindent{\textcolor{#1}{/* #2 */}}\Comment[#1]{// #3}}

\newcommand{\daniele}[1]{\ucomment{cyan}{#1}{DF}}

\newcommand{\SendCtx}{\textsc{SendCtx}}
\newcommand{\RetrieveCtx}{\textsc{RetrieveCtx}}
\newcommand{\RetrieveDict}{\textsc{RetrieveDict}}

\newcommand{\RetrieveParam}{\textsc{RetrieveParam}}

\newcommand{\SetAttr}{\textsc{SetAttr}}

\newcommand{\stored}{\mathsf{stored}}

\newcommand{\certattrs}{\mathcal{V}}
\newcommand{\attrcertifier}{AC}
\newcommand{\ctxs}{\mathsf{ctxs}}

\newcommand{\GFunc}{\mathcal{G}}
\newcommand{\policies}{\mathsf{pol}}

\newcommand{\advabe}{\advA_\formalMAABE}

\newcommand{\ignore}[1]{}

\newcommand{\attrcert}{\ensuremath{\mathit{AC}}}

==> addon/squeeze.tex <==
%% Saving trees -- put this in the preamble
\usepackage{times}
% Do not let the Times package affect the monospaced font (Courier is utterly ugly)
\renewcommand{\ttdefault}{cmtt}
%% Shrinking white space here and there…
% \usepackage[subtle]{savetrees}
\addtolength{\topmargin}{-1\baselineskip} % Caution!
\addtolength{\textheight}{2\baselineskip} % Caution!
%% save space around floats (tables, algo's, fig's):
% \setlength{\textfloatsep}{5pt}% Reduce \textfloatsep
%% save more space by suppressing vertical space between paragraphs
% \parskip0pt

==> tables/message-policies.tex <==
\begin{tabular}{|p{3.2cm}|c|p{0.5\columnwidth}|}
\hline
Message & Slice &  Policy \\ \hline
 \makecell{Supply purchase \\order (ramp)}
 &   & \lstinputlisting[firstline=1,lastline=1,linewidth=1.5\columnwidth]{code/policy.txt}\\ 
\hline
 \multirow{4}{*}{Export document}
 & \ref{item:intshipmentorder} &\lstinputlisting[firstline=2,lastline=2,linewidth=1.5\columnwidth]{code/policy.txt}\\ \cline{2-3}
 & \ref{item:csdd} &\lstinputlisting[firstline=3,lastline=3,linewidth=1.5\columnwidth]{code/policy.txt}\\ \cline{2-3}
 & \ref{item:orderreference} &\lstinputlisting[firstline=4,lastline=4,linewidth=1.5\columnwidth]{code/policy.txt}\\ \cline{2-3} 
 & \ref{item:invoice} &\lstinputlisting[firstline=5,lastline=5,linewidth=1.5\columnwidth]{code/policy.txt} \\
 \hline
 \makecell{National customs \\clearance}
 &   & \lstinputlisting[firstline=6,lastline=6,linewidth=1.5\columnwidth]{code/policy.txt} \\ \hline
\end{tabular}
